ChronoMagic-Bench: A Benchmark for Metamorphic Evaluation of Text-to-Time-lapse Video Generation

We propose a novel text-to-video (T2V) generation benchmark, ChronoMagic-Bench, to evaluate the temporal and metamorphic capabilities of the T2V models (e.g. Sora and Lumiere) in time-lapse video generation. In contrast to existing benchmarks that focus on visual quality and textual relevance of generated videos, ChronoMagic-Bench focuses on the model's ability to generate time-lapse videos with significant metamorphic amplitude and temporal coherence. The benchmark probes T2V models for their physics, biology, and chemistry capabilities, in a free-form text query. For these purposes, ChronoMagic-Bench introduces 1,649 prompts and real-world videos as references, categorized into four major types of time-lapse videos: biological, human-created, meteorological, and physical phenomena, which are further divided into 75 subcategories. This categorization comprehensively evaluates the model's capacity to handle diverse and complex transformations. To accurately align human preference with the benchmark, we introduce two new automatic metrics, MTScore and CHScore, to evaluate the videos' metamorphic attributes and temporal coherence. MTScore measures the metamorphic amplitude, reflecting the degree of change over time, while CHScore assesses the temporal coherence, ensuring the generated videos maintain logical progression and continuity. Based on ChronoMagic-Bench, we conduct comprehensive manual evaluations of ten representative T2V models, revealing their strengths and weaknesses across different categories of prompts, and providing a thorough evaluation framework that addresses current gaps in video generation research. Moreover, we create a large-scale ChronoMagic-Pro dataset, containing 460k high-quality pairs of 720p time-lapse videos and detailed captions ensuring high physical pertinence and large metamorphic amplitude. [Homepage](https://pku-yuangroup.github.io/ChronoMagic-Bench/).

==> content/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In the Appendix Section \ref{ethics_statement}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNo{Not include theoretical results}
	\item Did you include complete proofs of all theoretical results?
    \answerNo{Not include theoretical results}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{In the footnote of the Abstract and Appendix Section \ref{ethics_statement}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{In the Appendix Section \ref{ethics_statement}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{In the Appendix Section \ref{ethics_statement}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{In the Appendix Section \ref{ethics_statement}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{In the Appendix Section \ref{ethics_statement}.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{In the Appendix Section \ref{ethics_statement}.}
\end{enumerate}

\end{enumerate}

==> tables/table_OpenSoraPlan_comparison.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Quantitative comparison of OpenSoraPlan v1.1 \cite{opensoraplan} before and after fine-tuning using ChronoMagic-Pro.} "$\downarrow$" denotes lower is better. "$\uparrow$" denotes higher is better.}
    \label{table_opensoraplan_comparison}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{ccccccc}
        \toprule
        \textbf{Method} & \textbf{Venue} & \textbf{UMT-FVD$\downarrow$} & \textbf{UMTScore$\uparrow$} & \textbf{MTScore$\uparrow$} & \textbf{CHScore$\uparrow$} & \textbf{GPT4o-MTScore$\uparrow$} \\
        \midrule
        OpenSoraPlan v1.1 & Github'24 & 188.53 & 2.421 & 0.327 & 23.15 & 2.19 \\
        OpenSoraPlan v1.1 + ChronoMagic-Pro 10K + simple finetune & ours & 185.72 & 2.753 & 0.341 & 15.62 & 3.03 \\
        OpenSoraPlan v1.1 + ChronoMagic-Pro 10K + magictime finetune & ours & \textbf{180.11} & \textbf{2.864} & \textbf{0.346} & \textbf{25.72} & \textbf{3.05} \\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> tables/table_search_categories.tex <==
\begin{table}[!ht]
    \centering
    \caption{123}
    \begin{tabular}{c|c|c|c}
    \toprule
        \textbf{biological} & \textbf{human creation} & \textbf{meteorological} & \textbf{physical } \\ \midrule
        Blooming & Painting & Tide & Corrosion  \\ 
        Seed Growing & Construction & Solar Eclipse & Melting  \\ 
        ... & ... & ... & ...  \\
        ... & ... & ... & ...  \\
        Plant Dying & Fireworks & Day to Night & Explosion  \\ 
        Egg Hatching & 3D Printing & Rainbow Forming & Cooking  \\ \bottomrule
    \end{tabular}
    \label{table_search_categories}
\end{table}
